Pile of Law: Learning Responsible Data Filtering from the Law and a 256GB Open-Source Legal Dataset

One concern with the rise of large language models lies with their potential for significant harm, particularly from pretraining on biased, obscene, copyrighted, and private information. Emerging ethical approaches have attempted to filter pretraining material, but such approaches have been ad hoc and failed to take context into account. We offer an approach to filtering grounded in law, which has directly addressed the tradeoffs in filtering material. First, we gather and make available the Pile of Law, a 256GB (and growing) dataset of open-source English-language legal and administrative data, covering court opinions, contracts, administrative rules, and legislative records. Pretraining on the Pile of Law may help with legal tasks that have the promise to improve access to justice. Second, we distill the legal norms that governments have developed to constrain the inclusion of toxic or private content into actionable lessons for researchers and discuss how our dataset reflects these norms. Third, we show how the Pile of Law offers researchers the opportunity to learn such filtering rules directly from the data, providing an exciting new research direction in model-based processing.

==> old/0_introduction.tex <==
\section{Introduction}

The presence of undesirable content in the most popular corpora for pretraining large language models is a well-known fact. But what to do about it is largely a matter of researcher discretion. Some teams implement extensive processes for filtering content deemed toxic; others provide data in virtually unmodified form, relying only on dedpulication to preserve the utility of the data for training. 

There are two potential explanations for why filtering undesirable content has proven so difficult and uneven. First, it is practically difficult to perform reliable and transparent filtering at scale. That is partially because undesirable content is deeply contextual. For example, whether the inclusion of a racial epithet in a dataset is ``toxic'' may depend on factors such as the identity of the speaker and
% such as whether the epithet was `used' or `mentioned,' or 
the expectations of the readers \citep{ford2021racial, sperber1981irony}. 
% Filtering out all mentions of toxic content may harm 
Likewise, the existence of privacy violations may depend in part on the extent to which a speaker expected a fact to be widely shared at the time it was expressed \citep[6-7]{brown2022mean}. All of these expectations are constantly in flux and vary widely across countries \citep{bellman2004international}. 

Second, any filtering process imposes important tradeoffs. For example, imposing differential privacy standards on data may have severe adverse effects on its utility for applications serving important public goals \citep{ruggles2019differential}. Similarly, filtering may have unexpected effects on representation in datasets or the bias of downstream outputs \citep{dodge2021documenting, gururangan2022whose}. \cite{bagdasaryan2019differential} suggests that implementing the popular differential privacy framework can have a disparate impact on minority users. In short, researchers may find it hard to land on a principled approach to filtering toxic or private content when doing so means balancing competing interests.

This paper offers an alternative approach grounded in the law. Like other written data, legal and other government documents often contain private or offensive information. Governments have developed diverse standards for handling the trade-offs between privacy and offense on the one hand and transparency, access, and completeness on the other. 

We make two contributions. 

First, we provide researchers with a catalogue of the rules that apply to government documents. These rules often diverge from common practice. For example, despite the frequent reliance of researchers on lists of toxic words, we show that virtually all government norms permit the mention of racial epithets and the description of sexually explicit content in certain contexts. Word lists may thus be overinclusive. On the other hand, we show in Section 2 that there appears to be broad consensus across many jurisdictions that minors have a right against being identified in government records. To our knowledge, there has been less attention paid to the particular problem of protecting minors' identities in scraped web data. 

Many of the content inclusion rules we describe, however, are not bright-line tests, but rather require knowledge of context and local norms that may be difficult to encode via heuristics. Our second contribution is therefore to suggest that corpora consisting of government records can be used to calibrate heuristics to practices in a given jurisdiction. We demonstrate the power of this approach in two ways. In the context of privacy, we show that a commonly-used heuristic used to check for confidential medical information frequently flags de-identified public records from veterans' benefit claims that are \textit{a priori} known to comply with relevant privacy laws. In the context of toxicity, we show that frequently-used content filters likewise return many false positives from permissible uses of unsavory language. In short, researchers who wish to encode the nuanced privacy and toxicity rules developed by governments can do so directly by treating government data as a training environment.

To be clear up front, our argument is not that the rules developed for use in government and legal contexts are beyond reproach. To the contrary: The fact that different jurisdictions have developed different privacy standards suggests that there may be several defensible ways of balancing privacy and toxicity against other values. Indeed, we emphasize below that even \textit{within} countries approaches vary significantly, as for example in the case of access to juvenile criminal records across American states. In short, we offer no guarantee of optimality. What administrative rules \textit{do} provide, however, are a set of procedural guarantees about the provenance of a particular vector of decisions, based in the procedural fairness of the institutions that promulgated it. That is, while one cannot be sure that rules passed by the U.S. Congress are optimal, one \textit{can} be sure that they are the product of a procedure with some degree of democratic control. We believe that this is a significant improvement over unrestrained researcher discretion.




==> old/1_related_work.tex <==
\section{Related Work}


\subsection{The Challenge of Ethical Dataset Curation}

\subsubsection{Privacy}
Despite the growing focus on privacy in NLP (see \cite{brown2022mean} for a review), many major pre-training papers abandon any effort to explicitly filter private content. Not one of the papers reported in Table~\ref{tab:lit_review} includes a filtering step designed to protect against the inclusion of private content, despite taking a number of steps to filter other kinds of undesirable material. For example, although \cite{gao2020pile} excludes a number of data sources due to concerns that they could contain sexually explicit or racially derogatory content, they make no effort to assess the prevalence of potentially identifiable content within the dataset, despite including many natural-language sources (e.g. OpenWebText) in which users may have generated text with an expectation of anonymity. 

Instead, researchers have focused their attention on alternatives to filtering large aggregations of potentially sensitive text. \cite{kandpal2022dedupe} suggest that deduplication can have important benefits for protecting the privacy of data in pretraining corpora, and indeed deduplication is widely implemented by the papers in Table~\ref{tab:lit_review}. Federated learning side-steps concerns over aggregation by distributing training \cite{shokri2015privacy, hard2018federated}. Even under federated learning, however, the potential for information leakage remains. Learned model parameters such as embeddings \citep[e.g., ][]{songraghunathan2020leakage} or hidden representations \citep[e.g.,][]{coavoux2018repn} can be used to recover confidential information in the underlying text. And of course generative models can be prompted to reproduce the confidential information on which they were trained \citep{carlini2021extracting, carlini2019secret, bender2021dangers}. 

Thus, researchers have proposed a wide variety of approaches to modifying model training or outputs to protect against the leakage of private information at inference time. One approach, proposed by \cite{coavoux2018repn} and \cite{li2018robust}, is to add privacy objectives to the training regime, for instance in an adversarial learning framework. Alternatively, an approach grounded in differential privacy is to add localized noise to learned text representations \citep{lyu2020differentially, feyisetan2020challenges}, to apply other transformations to text at the encoding phase \citep{krishna2021adept, yue2021differential}, or to add noise to gradients \citep{mcmahan2018general}. 

These frameworks assume that the underlying dataset is private and disaggregated, for instance when a hospital transmits a health record for predictive inference about disease. It is trivial to see that they are less helpful when the underlying training data is known, aggregated, and public. For example, the inadvertent inclusion of social security numbers or other private facts in a publicly-accessible dataset would permit attackers to simply search the data themselves instead of deducing authorship information from model parameters. 

Thus, recent advances in deduplication and in protecting user privacy during training and inference do not relieve researchers assembling curated massive text datasets of responsibility for considering explicit filters for PII. Nor does the public-facing provenance of pre-training data negate any privacy interest that users may have. \textbf{[Elaborate on how aggregation and preservation can give rise to privacy interests].} Creators have a limited ability to mitigate harms stemming from the inclusion of harmful content once data sets have been released. \cite{peng2021mitigating}.

But how to implement that principle is unclear. One approach proposed by \cite{yue2021differential} is that corpora should be sanitized via the addition of noise to uncommon tokens that are detected in training data. [add more stuff about sanitizing from the Brown review]. Below, we offer an approach to sanitizing corpora grounded in legal principles. 

\subsubsection{Toxicity}



% \subsection{Other Legal Corpora}

% A number of prior works have pretrained smaller models on smaller subsets of legal data~\citep{chalkidis2020legal,zheng2021does}. None of these have conducted an analysis of the legal data itself or have curated a legal-focused pre-training dataset at this scale.


==> tables/toxicity_summary.tex <==
\begin{table}[]
\setlength{\tabcolsep}{4pt} % General space between cols (6pt standard)

    \centering
    \caption{Legal Norms Concerning Toxicity}
    \begin{tabular}{p{0.2\linewidth} p{0.45\linewidth}p{0.2\linewidth}p{0.15\linewidth}}
    \toprule
    \textbf{Category} & \textbf{Example} & \textbf{Rule} & \textbf{Appearance in Pile of Law }\\ 
           \midrule
       Epithet (Use) & ``I don't want any persons of [MASK] ancestry here.''   & Strictly Prohibited & Very rare. \\
      Epithet (Mention)  &  Reference to a discriminatory law in a case striking it down. & Allowed. & Frequent. \\ 
       Overt Bias  & Questioning why a sexual assault victim failed to resist in open court \citep{downesvbidwell} & Sanctioned  & Rare.\\
       Unconscious Bias  & Harsher language to describe crimes committed by members of a group. & Rarely sanctioned. & Frequent. \\ 
       Burdensome Effect & Argument that harms minorities.  & Allowed. & Frequent. \\ 
       \bottomrule
    \end{tabular}
    \label{tab:overt}
\end{table}


